Scoped Capabilities for Polymorphic Effects

Type systems usually characterize the shape of values but not their free variables. However, many desirable safety properties could be guaranteed if one knew the free variables captured by values. We describe CCsubBox, a calculus where such captured variables are succinctly represented in types, and show it can be used to safely implement effects and effect polymorphism via scoped capabilities. We discuss how the decision to track captured variables guides key aspects of the calculus, and show that CCsubBox admits simple and intuitive types for common data structures and their typical usage patterns. We demonstrate how these ideas can be used to guide the implementation of capture checking in a practical programming language.

==> alltyping.tex <==
\begin{figure*}[p!]
  % NOTE: this removes the page number, but also the conference name and line numbers
  %\thispagestyle{empty}

  \begin{minipage}{\textwidth}

  %\judgement{\textsf{Syntax}}{}
  %\vspace{-0.3em}

  \begin{minipage}{0.50\textwidth}
  \[
  \begin{array}[t]{llll@{\hspace{8mm}}l}
  \bbox{Value} & v, w & ::= & \lambda(x : T)t & \mbox{abstraction} \\
  && \OR & \lambda[X \sub R]t & \mbox{type abstraction} \\
  && \OR & \Boxed{x} & \mbox{boxing} \\[\medskipamount]

  \bbox{Answer} & a & ::= & v & \\
                   && \OR & x & \mbox{variable} \\[\medskipamount]

  \bbox{Term} &s, t& ::= & a & \\
        && \OR & x\,y & \mbox{application} \\
        && \OR & x\,[R] & \mbox{type application} \\
        && \OR & \Unboxed{C}{x} & \mbox{unboxing} \\
        && \OR & \Let{x: T}{s}{t} & \mbox{let}
  \end{array}
  \]
  \end{minipage}
  \begin{minipage}{0.50\textwidth}
  \[
  \begin{array}[t]{llll@{\hspace{8mm}}l}
  \bbox{Pure Type} & P, R & ::= & X & \mbox{type variable} \\
    && \OR & \Top & \mbox{top type} \\
    && \OR & \forall(x : S) T & \mbox{term function} \\
    && \OR & \forall[X \sub R] T & \mbox{type function} \\
    && \OR & \Boxed{T} & \mbox{boxed type} \\[\medskipamount]

  \bbox{Type} & S, T, U & ::= & R & \\
    && \OR & \Capt{C}{R} & \mbox{capturing type} \\[\medskipamount]

  \bbox{Capture set} & C, D & ::= & \{x_1, \ldots, x_n\} \\[\medskipamount]

  \bbox{Store context} & \sigma& ::= & \multicolumn{2}{l}{[\,] \ \OR\ \Let{x: T}{v}{\sigma}} \\
  \bbox{Eval context}  & e &::=& \multicolumn{2}{l}{[\,] \ \OR\ \Let{x: T}{e}{t}}
  \end{array}
  \]
  \end{minipage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}

  \judgement{Subcapturing}{\fbox{$\Gamma \ts C \sub C$}}

  \vspace{0.8em}
  \begin{minipage}{0.4\textwidth}
  \infrule[\ruledef{sc-set}]{%
    \Gamma \ts \cset{x_1} \sub C \ \ldots\ \Gamma \ts \cset{x_n} \sub C
  }{%
    \Gamma \ts \cset{x_1, \ldots, x_n} \sub C}
  \end{minipage}
  \begin{minipage}{0.35\textwidth}
  % \vspace{-1.5em}
  \infrule[\ruledef{sc-var}]{%
    x : \Capt{C_1}{R} \in \Gamma \quad
    \Gamma \ts C_1 \sub C_2
  }{%
    \Gamma \ts \cset{x} \sub C_2}
  \end{minipage}
  \begin{minipage}{0.24\textwidth}
    \vspace{-0.2em}
    \infrule[\ruledef{sc-elem}]{x \in C}{\Gamma \ts \cset{x} \sub C}
  \end{minipage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}

\judgement{Subtyping}{\fbox{$\Gamma \ts T \sub T$}}

  \begin{minipage}{0.5\textwidth}
  \infax[\ruledef{refl}]{%
    \Gamma \ts T \sub T
  }

  \vspace{0.8em}
  \infrule[\ruledef{tvar}]{%
    X \sub R \in \Gamma
  }{%
    \Gamma \ts X \sub R}

  \vspace{0.8em}
  \infrule[\ruledef{fun}]{%
    \Gamma \ts S_2 \sub S_1 \gap
    \Gamma, x: S_2 \ts T_1 \sub T_2
  }{%
    \Gamma \ts \forall(x: S_1)T_1 \sub \forall(x: S_2)T_2}

  \vspace{0.8em}
  \infrule[\ruledef{capt}]{%
    \Gamma \ts C_1 \sub C_2 \gap
    \Gamma \ts R_1 \sub R_2
  }{%
    \Gamma \ts \Capt{C_1}{R_1} \sub \Capt{C_2}{R_2}}



  \end{minipage}
  \begin{minipage}{0.5\textwidth}

  \infrule[\ruledef{trans}]{%
    \Gamma \ts T_1 \sub T_2 \gap \Gamma \ts T_2 \sub T_3
  }{%
    \Gamma \ts T_1 \sub T_3
  }
  \vspace{0.8em}

  \infax[\ruledef{top}]{%
    \Gamma \ts R \sub \top}

  \vspace{0.8em}
  \infrule[\ruledef{tfun}]{%
    \Gamma \ts R_2 \sub R_1 \gap
    \Gamma, x: R_2 \ts T_1 \sub T_2
  }{%
    \Gamma \ts \forall[X \sub R_1]T_1 \sub \forall[X \sub R_2]T_2}

  \vspace{0.8em}
  \infrule[\ruledef{boxed}]{%
    \Gamma \ts T_1 \sub T_2
  }{%
    \Gamma \ts \Boxed{T_1} \sub \Boxed{T_2}}

  \end{minipage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}

  \judgement{\textsf{Typing}}{\fbox{$\Gamma \ts t \typ T$}}

  \begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{var}]{%
    x: \Capt{C}{R} \in \Gamma
  }{%
    \Gamma \ts x \typ \Capt{\{x\}}{R}}

  \vspace{0.8em}
  \infrule[\ruledef{abs}]{%
    \Gamma, x: S \ts t: T
  }{%
    \Gamma \ts \lambda(x: S)t \typ \Capt{\cv(t)\backslash x}{\forall(x: S)T}}

  \vspace{0.8em}
  \infrule[\ruledef{app}]{%
    \Gamma \ts x \typ \Capt{C}{\forall(z: S)T} \gap
    \Gamma \ts y \typ S
  }{%
    \Gamma \ts x\,y \typ [z \mapsto y]T}

  \vspace{0.8em}
  \infrule[\ruledef{box}]{%
    \Gamma \ts x \typ \Capt{C}{R} \gap
    C \subseteq \dom(\Gamma)
  }{%
    \Gamma \ts \Boxed{x} \typ \Boxed{\Capt{C}{R}}}


  \vspace{0.8em}
  \infrule[\ruledef{let}]{%
    \Gamma \ts s: S \gap \Gamma, x: S \ts t: T \gap x \notin \fv(T)
  }{%
    \Gamma \ts \Let{x: S}{s}{t} : T}


  \end{minipage}
  \begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{sub}]{%
    \Gamma \ts t \typ S
    \gap
    \Gamma \ts S \sub T
    \gap
    \Gamma \ts T \wf
  }{%
    \Gamma \ts t \typ T }

  \vspace{0.8em}
  \infrule[\ruledef{tabs}]{%
    \Gamma, X \sub R \ts t: T
  }{%
    \Gamma \ts \lambda[X \sub R]t \typ \Capt{\cv(t)}{\forall[X \sub R]T}}

  \vspace{0.8em}
  \infrule[\ruledef{tapp}]{%
    \Gamma \ts x \typ \Capt{C}{\forall[X \sub R]T}
  }{%
    \Gamma \ts x\,[R] \typ [X \mapsto R]T}

  \vspace{0.8em}
  \infrule[\ruledef{unbox}]{%
    \Gamma \ts x \typ \Boxed{\Capt{C}{R}} \gap
    C \subseteq \dom(\Gamma)
  }{%
    \Gamma \ts \Unboxed{C}{x} \typ \Capt{C}{R}}

  \vspace{3em}
  \end{minipage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}

\judgement{Evaluation}{\fbox{$\Gamma \ts t \reduces t'$}}
% TODO: apparently we can't add labels (i.e. we can't link to the rules here),
% because we can only define one label per array. See:
% https://tex.stackexchange.com/questions/9939/multiply-defined-labels-using-hyperref
\[
\begin{array}{lclll}
  \storeof{\evalof{x\,y}}  &\reduces& \storeof{\evalof{[z \mapsto y]t}} & \gap \IF\ \sigma(x) = \lambda(z: T)t & \mbox{\sc (apply)} \\
  \storeof{\evalof{x\,[R]}}   &\reduces& \storeof{\evalof{[X \mapsto R]t}} & \gap \IF\ \sigma(x) = \lambda[X<:R']t & \mbox{\sc (tapply)} \\
  \storeof{\evalof{\Unboxed{C}{x}}} &\reduces& \storeof{\evalof{y}} & \gap \IF\ \sigma(x) = \Boxed{y} & \mbox{\sc (open)} \\
  \storeof{\evalof{\Let{x: T}{y}{t}}} &\reduces& \storeof{\evalof{[x \mapsto y]t}} && \mbox{\sc (rename)} \\
  \storeof{\evalof{\Let{x: T}{v}{t}}} &\reduces& \storeof{\Let{x: T}{v}{\evalof{t}}} & \gap \IF\ e \neq [\,] & \mbox{\sc (lift)} \\
  % \storeof{\evalof{t}} &\reduces& \storeof{\evalof{t'}} & \gap \IF\ \storeof{t} \reduces \storeof{t'}\gap & \mbox{\sc (context)}
\end{array}
\]

\comment{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}

  \judgement{\textsf{Well-formedness} \mbox{(in addition to \fsub rules)}}{\fbox{$\Gamma \ts t \wf$}}
  \vspace{0.8em}

  \begin{minipage}{0.5\textwidth}

  \infrule[\ruledef{capt-wf}]{%
    \Gamma \ts R \wf \gap C \subseteq dom(\Gamma) \cup \{\ccap\}
  }{%
  \Gamma \ts \Capt{C}{R} \wf}

  \end{minipage}
  \begin{minipage}{0.5\textwidth}

    \infrule[\ruledef{boxed-wf}]{%
      \Gamma \ts R \wf \gap C \subseteq dom(\Gamma)
    }{%
    \Gamma \ts \Boxed\Capt{C}{R} \wf}
  \end{minipage}
}
\end{minipage}
\caption{\label{fig:cc} System \CC}
\end{figure*}

==> reduction.tex <==
\begin{figure*}
% TODO: apparently we can't add labels (i.e. we can't link to the rules here),
% because we can only define one label per array. See:
% https://tex.stackexchange.com/questions/9939/multiply-defined-labels-using-hyperref
\[
\begin{array}{lclll}
  \storeof{\evalof{x\,y}}  &\reduces& \storeof{\evalof{[z \mapsto y]t}} & \quad \IF\ \sigma(x) = \lambda(z: T)t & \mbox{\sc (apply)} \\
  \storeof{\evalof{x\,[R]}}   &\reduces& \storeof{\evalof{[X \mapsto R]t}} & \quad \IF\ \sigma(x) = \lambda[X<:R']t & \mbox{\sc (tapply)} \\
  \storeof{\evalof{\Unboxed{C}{x}}} &\reduces& \storeof{\evalof{y}} & \quad \IF\ \sigma(x) = \Boxed{y} & \mbox{\sc (open)} \\
  \storeof{\evalof{\Let{x: T}{y}{t}}} &\reduces& \storeof{\evalof{[x \mapsto y]t}} && \mbox{\sc (rename)} \\
  \storeof{\evalof{\Let{x: T}{v}{t}}} &\reduces& \storeof{\Let{x: T}{v}{\evalof{t}}} & \quad \IF\ e \neq [\,] & \mbox{\sc (lift)} \\
  % \storeof{\evalof{t}} &\reduces& \storeof{\evalof{t'}} & \gap \IF\ \storeof{t} \reduces \storeof{t'}\gap & \mbox{\sc (context)}
\end{array}
\]

\caption{\label{fig:reduction} Evaluation Rules of System \CC}
\end{figure*}


==> subtyping.tex <==
\begin{figure*}
\small

  \judgement{Subcapturing}{\fbox{${\Gamma \ts C \sub C}$}}

  \vspace{0.8em}

  \begin{minipage}{0.3\textwidth}
    \infrule[\ruledef{sc-elem}]{x \in C}{\Gamma \ts \cset{x} \sub C}
  \end{minipage}
  \begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{sc-set}]{%
    \Gamma \ts \cset{x_1} \sub C \ \ldots\ \Gamma \ts \cset{x_n} \sub C
  }{%
    \Gamma \ts \cset{x_1, \ldots, x_n} \sub C}
  \end{minipage}

  \vspace{0.8em}

  \begin{minipage}{0.35\textwidth}
  \infrule[\ruledef{sc-var}]{%
    x : \Capt{C'}{S} \in \Gamma \quad
    \Gamma \ts C' \sub C
   }{%
     \Gamma \ts \cset{x} \sub C}
  \end{minipage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}


\judgement{Subtyping}{\fbox{$\Gamma \ts T \sub T$}}
\vspace{0.8em}

  \begin{minipage}{0.5\textwidth}
  \infax[\ruledef{refl}]{%
    \Gamma \ts T \sub T
  }

  \vspace{0.8em}
  \infrule[\ruledef{tvar}]{%
    X \sub S \in \Gamma
  }{%
    \Gamma \ts X \sub S}

  \vspace{0.8em}
  \infrule[\ruledef{fun}]{%
    \Gamma \ts U_2 \sub U_1 \gap
    \Gamma, x: U_2 \ts T_1 \sub T_2
  }{%
    \Gamma \ts \forall(x: U_1)T_1 \sub \forall(x: U_2)T_2}

  \vspace{0.8em}
  \infrule[\ruledef{capt}]{%
    \greyed{\Gamma \ts C_1 \sub C_2 \gap
    \Gamma \ts R_1 \sub R_2}
  }{%
    \greyed{\Gamma \ts \Capt{C_1}{R_1} \sub \Capt{C_2}{R_2}}}
  \end{minipage}\begin{minipage}{0.5\textwidth}

  \infrule[\ruledef{trans}]{%
    \Gamma \ts T_1 \sub T_2 \gap \Gamma \ts T_2 \sub T_3
  }{%
    \Gamma \ts T_1 \sub T_3
  }
  \vspace{0.8em}

  \infax[\ruledef{top}]{%
    \Gamma \ts S \sub \top}

  \vspace{0.8em}
  \infrule[\ruledef{tfun}]{%
    \Gamma \ts R_2 \sub R_1 \gap
    \Gamma, x: R_2 \ts T_1 \sub T_2
  }{%
    \Gamma \ts \forall[X \sub R_1]T_1 \sub \forall[X \sub R_2]T_2}

  \vspace{0.8em}
  \infrule[\ruledef{boxed}]{%
    \greyed{\Gamma \ts T_1 \sub T_2}
  }{%
    \greyed{\Gamma \ts \Boxed{T_1} \sub \Boxed{T_2}}}

  \end{minipage}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.3em}
\begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
\vspace{0.3em}

  \judgement{\textsf{Typing}}{\fbox{$\Gamma \ts t \typ T$}}

  \vspace{0.8em}
  \begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{var}]{%
    x: \Capt{\greyed C}{S} \in \Gamma
  }{%
    {\Gamma \ts x \typ \Capt{\greyed{\{x\}}}{S}}}

  \vspace{0.8em}
  \infrule[\ruledef{abs}]{%
    \Gamma, x: U \ts t: T
  }{%
    \Gamma \ts \lambda(x: U)t \typ \Capt{\greyed{\cv(t)\backslash x}}{\forall(x: U)T}}

  \vspace{0.8em}
  \infrule[\ruledef{app}]{%
    \Gamma \ts x \typ \Capt{\greyed C}{\forall(z: U)T} \gap
    \Gamma \ts y \typ U
  }{%
    \Gamma \ts x\,y \typ [z \mapsto y]T}

  \vspace{0.8em}
  \infrule[\ruledef{box}]{%
    \greyed{\Gamma \ts x \typ \Capt{C}{S} \gap
    C \subseteq \dom(\Gamma)}
  }{%
    \greyed{\Gamma \ts \Boxed{x} \typ \Boxed{\Capt{C}{S}}}}

  \end{minipage}\begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{sub}]{%
    \Gamma \ts t \typ T
    \gap
    \Gamma \ts T \sub U
    \gap
    \Gamma \ts U \wf
  }{%
    \Gamma \ts t \typ U }

  \vspace{0.8em}
  \infrule[\ruledef{tabs}]{%
    \Gamma, X \sub S \ts t: T
  }{%
    \Gamma \ts \lambda[X \sub S]t \typ \Capt{\greyed{\cv(t)}}{\forall[X \sub S]T}}

  \vspace{0.8em}
  \infrule[\ruledef{tapp}]{%
    \Gamma \ts x \typ \Capt{\greyed C}{\forall[X \sub S]T}
  }{%
    \Gamma \ts x\,[S] \typ [X \mapsto S]T}

  \vspace{0.8em}
  \infrule[\ruledef{unbox}]{%
    \greyed{\Gamma \ts x \typ \Boxed{\Capt{C}{S}} \gap
    C \subseteq \dom(\Gamma)}
  }{%
    \greyed{\Gamma \ts \Unboxed{C}{x} \typ \Capt{C}{S}}}
  \end{minipage}


  \vspace{0.8em}
  \begin{minipage}{0.5\textwidth}
    \infrule[\ruledef{let}]{%
    \Gamma \ts s: T \gap \Gamma, x: T \ts t: U \gap x \notin \fv(U)
  }{%
    \Gamma \ts \Let{x: T}{s}{t} : U}
  \end{minipage}

  \vspace{0.3em}
  \begin{center}\rule{0.9\textwidth}{0.4pt}\end{center}
  \vspace{0.3em}

  \judgement{Evaluation}{\fbox{$\Gamma \ts t \reduces t'$}}
  \vspace{0.8em}
  % TODO: apparently we can't add labels (i.e. we can't link to the rules here),
  % because we can only define one label per array. See:
  % https://tex.stackexchange.com/questions/9939/multiply-defined-labels-using-hyperref
  \[
  \begin{array}{lclll}
    \storeof{\evalof{x\,y}}  &\reduces& \storeof{\evalof{[z \mapsto y]t}} & \gap \IF\ \sigma(x) = \lambda(z: T)t & \mbox{\sc (apply)} \\
    \storeof{\evalof{x\,[S]}}   &\reduces& \storeof{\evalof{[X \mapsto S]t}} & \gap \IF\ \sigma(x) = \lambda[X<:S']t & \mbox{\sc (tapply)} \\
    \storeof{\evalof{\Unboxed{C}{x}}} &\reduces& \storeof{\evalof{y}} & \gap \IF\ \sigma(x) = \Boxed{y} & \mbox{\sc (open)} \\
    \storeof{\evalof{\Let{x: T}{y}{t}}} &\reduces& \storeof{\evalof{[x \mapsto y]t}} && \mbox{\sc (rename)} \\
    \storeof{\evalof{\Let{x: T}{v}{t}}} &\reduces& \storeof{\Let{x: T}{v}{\evalof{t}}} & \gap \IF\ e \neq [\,] & \mbox{\sc (lift)} \\
    % \storeof{\evalof{t}} &\reduces& \storeof{\evalof{t'}} & \gap \IF\ \storeof{t} \reduces \storeof{t'}\gap & \mbox{\sc (context)}
  \end{array}
  \]

  \begin{minipage}{\textwidth}
  {\bf \ \ \ where}
  $\begin{array}[t]{llll@{\hspace{8mm}}l}
  \bbox{Store context} & \sigma& ::= & \multicolumn{2}{l}{[\,] \OR \Let{x: T}{v}{\sigma}} \\
  \bbox{Eval context}  & e &::=& \multicolumn{2}{l}{[\,] \OR \Let{x: T}{e}{t}}
  \end{array}$
  \end{minipage}

\caption{\label{fig:cc-rules} Typing and Evaluation Rules of System \CC}
\end{figure*}


==> typing.tex <==
\begin{figure*}
  \begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{var}]{%
    x: \Capt{C}{R} \in \Gamma
  }{%
    \Gamma \ts x \typ \Capt{\{x\}}{R}}

  \vspace{0.8em}
  \infrule[\ruledef{abs}]{%
    \Gamma, x: S \ts t: T
  }{%
    \Gamma \ts \lambda(x: S)t \typ \Capt{\cv(t)\backslash x}{\forall(x: S)T}}

  \vspace{0.8em}
  \infrule[\ruledef{app}]{%
    \Gamma \ts x \typ \Capt{C}{\forall(z: S)T} \gap
    \Gamma \ts y \typ S
  }{%
    \Gamma \ts x\,y \typ [z \mapsto y]T}

  \vspace{0.8em}
  \infrule[\ruledef{box}]{%
    \Gamma \ts x \typ \Capt{C}{R} \gap
    C \subseteq \dom(\Gamma)
  }{%
    \Gamma \ts \Boxed{x} \typ \Boxed{\Capt{C}{R}}}


  \vspace{0.8em}
  \infrule[\ruledef{let}]{%
    \Gamma \ts s: S \gap \Gamma, x: S \ts t: T \gap x \notin \fv(T)
  }{%
    \Gamma \ts \Let{x: S}{s}{t} : T}


  \end{minipage}
  \begin{minipage}{0.5\textwidth}
  \infrule[\ruledef{sub}]{%
    \Gamma \ts t \typ S
    \gap
    \Gamma \ts S \sub T
    \gap
    \Gamma \ts T \wf
  }{%
    \Gamma \ts t \typ T }

  \vspace{0.8em}
  \infrule[\ruledef{tabs}]{%
    \Gamma, X \sub R \ts t: T
  }{%
    \Gamma \ts \lambda[X \sub R]t \typ \Capt{\cv(t)}{\forall[X \sub R]T}}

  \vspace{0.8em}
  \infrule[\ruledef{tapp}]{%
    \Gamma \ts x \typ \Capt{C}{\forall[X \sub R]T}
  }{%
    \Gamma \ts x\,[R] \typ [X \mapsto R]T}

  \vspace{0.8em}
  \infrule[\ruledef{unbox}]{%
    \Gamma \ts x \typ \Boxed{\Capt{C}{R}} \gap
    C \subseteq \dom(\Gamma)
  }{%
    \Gamma \ts \Unboxed{C}{x} \typ \Capt{C}{R}}

  \vspace{3em}
  \end{minipage}

\caption{\label{fig:typing} Typing Rules of System \CC}
\end{figure*}

